Graph Neural Networks for Multimodal Single-Cell Data Integration

Recent advances in multimodal single-cell technologies have enabled simultaneous acquisitions of multiple omics data from the same cell, providing deeper insights into cellular states and dynamics. However, it is challenging to learn the joint representations from the multimodal data, model the relationship between modalities, and, more importantly, incorporate the vast amount of single-modality datasets into the downstream analyses. To address these challenges and correspondingly facilitate multimodal single-cell data analyses, three key tasks have been introduced: $\textit{modality prediction}$, $\textit{modality matching}$ and $\textit{joint embedding}$. In this work, we present a general Graph Neural Network framework $\textit{scMoGNN}$ to tackle these three tasks and show that $\textit{scMoGNN}$ demonstrates superior results in all three tasks compared with the state-of-the-art and conventional approaches. Our method is an official winner in the overall ranking of $\textit{Modality prediction}$ from NeurIPS 2021 Competition, and all implementations of our methods have been integrated into DANCE package~\url{https://github.com/OmicsML/dance}.

==> sections/exp_back.tex <==
\setlength{\textfloatsep}{1pt}% Remove \textfloatsep
\section{Experiments}
In this section, we evaluate the effectiveness of our framework \method{} against three tasks and show how \method{} outperforms all other models over all three tasks by combining our general framework with task-specific design. In particular, we aim to answer the following two questions: \label{sec:q}
(1) How does \method{} perform compared to the other models on the leaderboard? Is our proposed graph neural networks framework well adapted to various tasks in single cell multimodal data integration?
(2) Do we really benefit from the graph structural information?


% In the following sections, we separately present the experimental settings of each subtask and the corresponding results. After all, we conduct ablation study and parameter analysis of \method{}, eventually answer the questions above. 


\subsection{Modality Prediction}
\subsubsection{Datasets} In the modality prediction dataset, each modality is provided with source data, preprecossed data (with default methods), and batch labels. The size of the dataset is shown in the Table~\ref{dataset_task1}. Note that the GEX-ATAC and ATAC-GEX subtasks are not entirely symmetric, because in GEX-ATAC task, the output dimension is deliberately reduced, where 10,000 ATAC features are randomly selected out of the original 116,490 dimensions.


In addition, it is allowed to conduct online training given the input modality of testing data, thus most teams using auto-encoders opted for fine-tuning on test data, while our graph neural networks enabled transductive learning.

\subsubsection{Settings and Parameters} 

For each experiment, we report the average performance of 10 runs. In each run, we randomly choose 85\% of cells from the training data for validation and the remaining 15\% of cells for validation. When the validation loss does not decrease within 300 epochs, the training is terminated, and the parameter with the best validation performance is adopted. 

Additionally, in practice, we utilized the initial residual instead of the skip connections in Eq.\ref{eq:v} used group normalization for aggregation results and dismissed the edge weight normalization stated in Eq.~\ref{eq:norm}, these two modifications empirically improved our performance while didn't change \method{} architecture. Besides, we manually set our parameter $\alpha$ in Eq.~\ref{eq:a} to $0.5$, specific effects of this parameter will be discussed in later sections. 
% Other hyper-parameter settings can be found in the appendix \hongzhi{appendix reference}.

\subsubsection{Baselines}
To be mentioned, in Table~f\ref{task1lb}, we only show the teams that acquired top results in one or more subtasks in the competition, because they are officially required to declare their model details. For further comparison, we briefly detail each method: (1) {Baseline}, a truncated-SVD dimsionality reduction followed by linear regression.
(2) {Dengkw}, a well-designed model based on kernel ridge regression.
(3) {Novel}, an encoder-decoder structure with LSI preprecessing.
(4) {Living System Lab}, an ensemble model composed of random forest models, catboost\cite{prokhorenkova2018catboost} models, and k-nearest neighbors regression models.
(5) {Cajal}, a feed foward neural network with heavy feature selections guided by prior knowledge.
(6) {ScJoint}, an ensembled neural network model incorporated various strategies of preprocessing such as extracting tf-idf features and filtering highly variable genes/features.



% \begin{itemize}
%     \item \textbf{Baseline}: A truncated-SVD dimsionality reduction followed by linear regression.
%     \item \textbf{Dengkw}: A well-designed model based on kernel ridge regression.
%     \item \textbf{Novel}: An encoder-decoder structure with LSI preprecessing (the same as we discussed in \ref{sec:lsi}).
%     \item \textbf{Living System Lab}: An ensemble model composed of random forest models, catboost\cite{prokhorenkova2018catboost} models, and k-nearest neighbors regression models.
%     \item \textbf{Cajal}: A feed foward neural network with heavy feature selections guided by prior knowledge.
%     \item \textbf{ScJoint}:  An ensembled neural network model incorporated various strategies of preprocessing such as extracting tf-idf features and filtering highly variable genes/features.
% \end{itemize}
 
The source codes for all the methods above can be found in the official github\footnote{\url{https://github.com/openproblems-bio/neurips2021_multimodal_topmethods}}. It can be seen that the existing models are relatively simple, mainly based on traditional machine learning models and autoencoders. In contrast, our framework has a more complicated structure, which leads to the flexibility to different structural data (e.g. graph data) and different tasks. This makes our framework a very suitable backbone in the field of single-cell multimodal data integration.

\subsubsection{Results}

As shown in Table~\ref{task1lb}, our methods achieved a lowest overall score in the competition (the lower, the better). An interesting phenomenon is that there is no team lead consistently across all subtasks, resulted in individual winner for each category, which is very different from the other two tasks. However, as far as we know, there is no team that focus on only one subtask. Such phenomenon may be caused by two reasons: (\textbf{i}) modality prediction task is the most competitive task in the competition, many participating teams only focused on this task (including our own team), as a result, over 40 individual teams appeared on the final leaderboard. Thus, it is not surprising that we have several winners. (\textbf{ii}) Modality prediction task has only 1,000 cells in the private testing dataset, therefore, certain variance exists in the evaluation results. However, the charm of the competition lies in the emphasis on the best result rather than the average performance, as a result, some particularly good results decide the winner. Compared to the other models, our GNN model presented a consistently good performance and became the overall winner in the competition.

Furthermore, we continued working on this task after the competition and made several modifications to our original models, including: a learning-rate decay training strategy, more hidden units along with stronger regularization of dropout and weight decay.  Eventually, we've effectively strengthened our graph neural network model hence significantly improved our results, especially in the toughest subtask GEX-to-ADT, where the output for each cell is a 134-dimensional dense vector, and we now achieved an rmse loss of $0.3809$ which is much lower than previous best score of $0.3854$ in the competition. Overall, the results prove the effectiveness of our GNN framework, and in some specific cases, \method{} have tremendous advantage in view of performance.


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[t]
\footnotesize
\caption{Performances for Modality Prediction (Task 1) \downarrow}
\begin{tabular}{lccccc}
\toprule
                                                                    & GEXADT                                                   & ADT2GEX                                                   & GEX2ATAC                                                  & ATAC2GEX                                                   & Overall \\ \midrule
Baseline                                                            & 0.4395                                                       & 0.3344                                                       & 0.1785                                                       & 0.2524                                                        & 0.3012  \\
Dengkw*                                                             & 0.3854                                                       & 0.3242                                                       & 0.1833                                                       & 0.2449                                                        & 0.2836  \\
Novel                                                               & 0.4153                                                       & $\bf 0.3177$                                                 & 0.1781                                                       & 0.2531                                                        & 0.2911  \\
LS. Lab*                                                            & 0.4065                                                       & 0.3228                                                       & $\bf 0.1774$                                                 & 0.2393                                                        & 0.2865  \\
Cajal                                                               & 0.4393                                                       & 0.3311                                                       & 0.1777                                                       & $\bf 0.2169$                                                  & 0.2891  \\
ScJoint*                                                            & 0.3954                                                       & 0.3247                                                       & 0.1785                                                       & 0.2377                                                        & 0.2840  \\ 
\method{} & 0.3898                                                       & 0.3221                                                       & 0.1776                                                       & 0.2403                                                        & 0.2824  \\ \midrule
\begin{tabular}[c]{@{}l@{}}\method{} \\ (Single)\end{tabular}       & \begin{tabular}[c]{@{}l@{}}0.3885\\ $\pm$0.0043\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.3242\\ $\pm$0.0018\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.1778\\ $\pm$0.0001\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.2399\\ $\pm$0.0013\end{tabular} & 0.2826  \\ \midrule
\begin{tabular}[c]{@{}l@{}}\method{}* \\ (Ensemble)\end{tabular}    & $\bf 0.3809$                                                 & 0.3223                                                       & 0.1777                                                       & 0.2392                                                        & $\bf 0.2800$  \\ \bottomrule
\end{tabular}
\label{task1lb}
%\vskip -1em
\end{table}


\subsection{Modality Matching}
\subsubsection{Datasets} The majority part of the modality matching dataset is the same as the modality prediction dataset (as shown in Table \ref{dataset_task2}, while several differences exist: (\textbf{i}) the cells in the testing dataset is much more than the previous task; (\textbf{ii}) GEX-ATAC and ATAC-GEX subtasks now become perfectly dual tasks; and (\textbf{iii}) in each modality, the order of cells is messed up; in the training data, the correspondence between two modalities is given in an extra file, while for the test data, we have no correspondence between the data, where our goal is to find a match.

\subsubsection{Settings and Parameters} \label{setting:match}
The experiment settings are similar to the previous task, while in practice, we make some adjustments again. For calculation convenience, we follow the recent practical trends in graph neural networks, to decouple the propagation and transformation. Although decoupled graph neural networks are not equivalent to the original coupled version, empirical results show that this simplified version of the graph neural network do not degrade the performance. 

It is worth noting that batch labels are given in company with the testing data, which provides a very strong prior knowledge for matching. More concretely, we can first divide the testing data into different batches, hence match the data that belong to the same batch. This method dramatically reduced the search space, result in a significant performance boost. To be fair, we have confirmed that the winner solution also used this strategy in the competition.


\subsubsection{Baselines}
The same as the previous section, in Table~f\ref{task2lb}, here we only show teams that acquired top results in one or more subtasks in the competition. Now we briefly introduce those models:
(1) {Baseline}, first project one modality to the other with linear regression, then search for the nearest neighbors in the same modality.
(2) {GLUE}, a variational auto-encoder (VAE) model supervised by three auxiliary losses. 
(3) {Novel}, a feed-forward neural network directly supervised by matching loss.


\subsubsection{Results}
As shown in Table~\ref{task2lb}, \method{} outperforms the winner team and the runner-up team with a very large margin. Note that we didn't create any models for this task during the competition, because of that we don't have any results on the official leaderboard.  

The score of the metric can be roughly understood as the accuracy of predicting a right correspondence for each piece of data, meanwhile the search space grows with the total number of cells in the testing data. For example, in testing phase of the ADT-to-GEX subtask, we have 15,066 cells to match, thus for each piece of ADT data, we have 15,066 candidates in GEX data. The mathematical expectation of the accuracy of randomly guess thus equals to $\frac{1}{15,066}$, which can be considered as an indicator of the task difficulty. From this point of view, \method{} already achieved very high performance (e.g. 0.08 in ADT-GEX subtask).

It is also worth noticing that both team Novel's model and \method{} utilizes a symmetric matching algorithm, thus we have exactly the same performance for dual subtasks (e.g. GEX2ADT and ADT2GEX). Another interesting point is that our proposed graph neural network model is especially good at GEX-ADT dual subtasks, where we improved the previous winning performance from 0.05 to 0.08 approximately. To understand why, a deeper analysis is required, yet we leave it for the future works.

% \begin{table*}[]
% \caption{Task 2 Modality Matching}
% \begin{tabular}{@{}lccccc@{}}
% \toprule
%  & GEX-to-ADT & ADT-to-GEX & GEX-to-ATAC & ATAC-to-GEX & Overall \\ \midrule
% Baseline & 0.0000 & 0.0000 & 0.0001 & 0.0001 & 0.0001 \\
% GLUE & 0.0495 & 0.0516 & 0.0560 & 0.0583 & 0.0539 \\
% Novel & 0.0373 & 0.0373 & 0.0412 & 0.0412 & 0.0392 \\ \midrule
% \method{} & ${\bf0.0810\pm0.0015}$ & ${\bf0.0810\pm0.0015}$ & ${\bf0.0630\pm0.0014}$  & ${\bf0.0630 \pm	0.0014}$ & \textbf{0.0720} \\ \midrule
% \end{tabular}
% \label{task2lb}
% \end{table*}

% Please add the following required packages to your document preamble:


\begin{table}[]
\caption{Performances for Modality Matching (Task 2)\uparrow}
\footnotesize
\begin{tabular}{@{}lccccc@{}}
\toprule
                           & GEX2ADT                                                            & ADT2GEX                                                            & GEX2ATAC                                                           & ATAC2GEX                                                           & Overall         \\ \midrule
Baseline                   & 0.0000                                                                & 0.0000                                                                & 0.0001                                                                & 0.0001                                                                & 0.0001          \\
GLUE                       & 0.0495                                                                & 0.0516                                                                & 0.0560                                                                & 0.0583                                                                & 0.0539          \\
Novel                      & 0.0373                                                                & 0.0373                                                                & 0.0412                                                                & 0.0412                                                                & 0.0392          \\ \midrule
\method{} & \textbf{\begin{tabular}[c]{@{}l@{}}0.0810\\ $\pm$0.0015\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}0.0810\\ $\pm$0.0015\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}0.0630\\ $\pm$0.0014\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}0.0630\\ $\pm$0.0014\end{tabular}} & \textbf{0.0720} \\ \bottomrule
\end{tabular}
\label{task2lb}
% \vskip -1em
\end{table}


	 			
\subsection{Joint Embedding}
\subsubsection{Datasets}
The training data of this task are basically the same as the modality prediction task, moreover, data from different modalities are already aligned. Additionally, cell type labels are also provided in training phase, while testing data consist of all the train cells and unseen test cells but are not along with cell type labels.

\subsubsection{Settings and Parameters}
Considering that the input in this task is very similar to modality matching, we follow \ref{setting:match} to decouple our graph neural networks model. %Other details can be found in \hongzhi{Appendix reference}.

\subsubsection{Baselines}
We briefly describe the other three models in Table~\ref{task3lb}:
(1) {Baseline}, a concatenation of PCA results of two modalities.
(2) {JAE}, an auto-encoder model that incorporates extra supervision (cell annotations).
(3) {GLUE}, an auto-encoder model guided by an external knowledge graph.

\subsubsection{Results}
As shown in Table~\ref{task3lb}, our \method{} significantly outperforms the other two models in GEX-ADT joint embedding task, with an improvement over 0.1 according to the average metric.


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[t]
\small
\caption{Performances for Joint Embedding (Task 3)\uparrow}
\begin{tabular}{@{}lccccccc@{}}
\cmidrule(r){1-8}
             & NMI cluster/label                      & Cell type ASW           & Cc\_con         & Traj\_con       & Batch ASW     & Graph connectivity           & Average metric           \\ \cmidrule(r){1-8}
Baseline     & 0.6408                   & 0.5266                   & \textbf{0.9270} & 0.8325          & 0.7982          & 0.8945                   & 0.7699                   \\
Amateur (JAE) & 0.7608                   & 0.6043                   & 0.7817          & \textbf{0.8631} & 0.8432          & 0.9700                   & 0.8039                   \\
GLUE         & 0.8022                   & 0.5759                   & 0.6058          & 0.8591          & \textbf{0.8800} & 0.9506                   & 0.7789                   \\ \cmidrule(r){1-8}
\method{}    & \textbf{0.8499 ± 0.0032} & \textbf{0.6496 ± 0.0046} & 0.7084 ± 0.0316 & 0.8532 ± 0.0019 & 0.8691± 0.0020  & \textbf{0.9708 ± 0.0041} & \textbf{0.8168 ± 0.0051} \\ \cmidrule(r){1-8}
\end{tabular}
\label{task3lb}
\vskip -1em
\end{table*}

\begin{figure}[t]%
     \centering
     \label{fig:x}{\includegraphics[width=0.7\linewidth]{figures/task2_ablation.pdf} }%
    \qquad
    \vskip -0.5em
\caption{Ablation study of modality matching task.}
\label{fig:abl}%
\end{figure}

\begin{figure}[t]%
     \centering
     \label{fig:x}{\includegraphics[width=0.7\linewidth]{figures/parameter.pdf} }%
    \qquad
    \vskip -0.5em
\caption{Parameter analysis of layer weight $\bf w$.}
\label{fig:prm}%
% \vskip -2em
\end{figure}


\subsection{Ablation Study}
Throughout the previous sections, we have examined that our graph nerual network general framework is suitable for all these tasks in single-cell multimodal data integration. Now we start to answer the other questions we raised at the beginning of Section~\ref{sec:q}. We choose modality matching task as an example, because in modality matching task we use decoupled GNN, we can easily remove the graph structural information by removing the propagation layers. The result is referred to as ``w/o propagation'' in Figure~\ref{fig:abl}. The performance significantly drop from $0.0810$ to $0.0745$ in GEX-ADT subtask and from $0.0630$ to $0.0562$ in GEX-ATAC respectively, showing that the graph structural information extracted by the propagation layers indeed helped a lot with our performance.

We also examined the importance of our auxiliary loss, also shown in Figure~\ref{fig:abl}. Without the supervision of auxiliary losses, \method{} lost a lot of generalization ability, behaving as poor as without graph structural information. Another minor issue we discuss here, is that some negative values exist in the adjacency matrix, causing by feature dimensionality reduction, which leads to the failure of conventional weight normalization methods. As an alternative, we proposed two solutions. One is to standardize results of the aggregation to replace the normalization of the adjacency matrix; the other is to use the min max scaling algorithm to project all the values on the adjacency matrix to $[0,1]$. The results show that the first solution slightly outperforms the second one, although there might exist other optimal solutions.

\subsection{Parameter Analysis}
We analyzed an important parameter in our framework, i.e. $\bf w$ in Eq.~\ref{eq:ro}, in order to bring a deeper insight on \method{}. Specifically, $\bf w$ is a learnable parameter that controls the weight between each propagation layer. To some extent, the value of $\bf w$ can prove to us the effectiveness of graph structural information and help us understand how much higher-order structural information is valued by models in different tasks. Therefore we show values of $\bf w$ learned by \method{} in different tasks in \ref{fig:prm}. Note that in different tasks we have different numbers of layers, in modality prediction task we have 4 layers and in modality matching task and joint embedding task we have 3 layers and 2 layers respectively. The results consistently show that \method{} tends to synthesize the information in each layer, not just limited to the shallow layer, which shows that the information of the higher-order graph structure is indeed effective. As for more details, joint embedding depends more on local information, which exists in source input data. While in modality prediction task, More higher-order information is referenced, indicating that the model needs to enrich more information from similar cells or similar features. This can be explained from the need for more detailed information in modality prediction. We 
believe we can unearth more meaningful information from the parameter
analysis, but we leave them to future work.

% 4.1
% \wei{ablation study; histogram plot.}

% \wei{parameter analysis: $\alpha$; number of layers;}

% \wei{weight plot for 3 tasks.}

% 4.2
% \wei{ablation study; histogram plot.}


% \subsection{Summary}
% \wei{need a section to summarize all the findings}

==> sections/intro_old.tex <==




% What is the problem, why GNN
\wei{First paragraph: prevalence and importance of single cell data; single-cell data integration, tasks.\hongzhi{finished}\\ Second paragraph: methods for the above tasks;  However, these methods have their limitations. (data noise; limited neighborhood size; )\\ Third paragraph: Recently, the advances of graph neural networks~\cite{} pave the way for overcoming the above limitations in single-cell data integration. Specifically, xxxx (what GNNs do and how it helps address the issues).  In addition, it is easy to incorporate external knowledge into the constructed graph and apply GNNs to exploit the additional structural information.   (We may also mention transductive learning which can help us gain additional  semi-supervised signal to enhance the representation learning process) \\ Fourth paragraph: Yet, designing GNNs for single-cell faces several crucial challenges: (1)(2)... To address these challenges, we propose to xxxxx. \\ Our contributions can be summarized as follows: 123, including  competition result}
\newpage

\section{Introduction}

\wei{technology-->data-->usefulness-->tasks}

\wei{Existing are developed for single; few attention xxx.}

\wei{limitations...}

\wei{gnn..}



The rapid development of single-cell technologies makes it possible to quickly and efficiently measure several features of cells at the same time.  For example, CITE-seq (cellular indexing of transcriptomes and epitopes by sequencing) enables joint quantification of RNA expression and protein markers~\cite{stoeckius2017simultaneous}; and Multiome Assay for Transposase-Accessible Chromatin (ATAC, i.e. genome-wide DNA accessibility) using sequencing  + Gene Expression, provides a view across all DNA and RNA in the cell~\cite{cao2018joint}. These multimodal joint measurement methods can provide multimodal aligned data which contributes to a more comprehensive view of the layers of genomics regulation. 

The advanced single-cell measurement technology has been driving a revolution in the life sciences. Taking advantage of diverse modalities ranging from gene expression and chromatin accessibility to proteomics, we are able to precisely characterize cellular states. However, the majority of existing techniques can measure only one modality for each cell at a single time (e.g. only the RNA sequence for each cell), which limited the study of the interaction between different layers of genomic regulation. Thus, more attention has been paid on the integration of different modalities ~\cite{rautenstrauch2021intricacies}. \jt{I think we need to add more references}%
%https://openproblems.bio/media/learning/differing\_expression.png
%
In the last few years, there was a big success in single-cell measurement technology to simultaneously measure multiple modalities (e.g. DNA, RNA, and protein accessibility) in the same cell~\cite{stuart2019integrative, ma2020integrative}.  For example, CITE-seq (cellular indexing of transcriptomes and epitopes by sequencing) enables joint quantification of RNA expression and protein markers~\cite{stoeckius2017simultaneous}; and Multiome Assay for Transposase-Accessible Chromatin (ATAC, i.e. genome-wide DNA accessibility) using sequencing  + Gene Expression, provides a view across all DNA and RNA in the cell~\cite{cao2018joint}. These multimodal joint measurement methods can provide multimodal aligned data which contributes to a more comprehensive view of the layers of genomics regulation. 



\wei{maybe we don't need to describe all three tasks here. just one task and describe its importance for multi-modality data}\jt{I think we need to give a few sentences about the motivation of the competition}In light of this, researchers from computational biology recently organized a competition, the Multimodal Single-Cell Data Integration competition at NeurIPS 2021\hongzhi{reference}. The competition includes three tasks, i.e., modality prediction, modality matching and joint embedding. The modality prediction task aims at predicting one modality from another modality (e.g. to predict protein markers from RNA expression). While the modality matching task focuses on identifying the correspondence between different modalities (e.g. given protein markers and RNA expression samples, to identify which samples belong to the same cell). The motivation of these two tasks is to better integrate existing single-cell datasets which mostly measure only one modality. Meanwhile, the joint embedding task aims to provide a comprehensive embedding for each single cell, which directly utilizes aligned data from different modalities. With the multimodal data, we can gain a deeper insight into the state of a cell, thus the joint embedding generated from multimodal data can better characterize cellular heterogeneity and serve downstream tasks.

%A number of recent works are related to these multimodal integration tasks. BABEL\cite{wu2021babel} translated between the transcriptome and chromatin profiles of a single cell based on an encoder-decoder architecture.  scMM\cite{minoura2021scmm} implemented a mixture-of-experts deep generative model for joint embedding learning and modality prediction. Cobolt\cite{gong2021cobolt} acquired joint embedding via a variant of Multimodal Variational Autoencoder (MVAE\cite{yao2021transcriptomic}). MOFA2\cite{argelaguet2020mofa+} used Bayesian group factor analysis to reduce dimensions of multi-modality data, thus also generate a low-dimensional joint representation. All these methods take advantage of integrated multimodal single-cell data.

There are recent works taking advantage of integrated multimodal single-cell data. BABEL\cite{wu2021babel} translated between the transcriptome and chromatin profiles of a single cell based on an encoder-decoder architecture;  scMM\cite{minoura2021scmm} implemented a mixture-of-experts deep generative model for joint embedding learning and modality prediction.  Cobolt\cite{gong2021cobolt} acquired joint embedding via a variant of Multimodal Variational Autoencoder (MVAE\cite{yao2021transcriptomic}). MOFA2\cite{argelaguet2020mofa+} used Bayesian group factor analysis to reduce dimensions of multi-modality data, thus also generate a low-dimensional joint representation. However,\jt{I think here we can put more details; otherwise it is very wired to directly mention high-order information.  I think we can say: they denote each cell as a high-dimensional and sparse vector and consider each cell as input. In such way, we can naturally mention that they do not consider high-order information among cells and the input is high-dimensional and sparse. We can use one of the compeition tasks as an example to illustrate what is the dimension and how sparse it is on average? we can draw a figure to illusrate the data and later on we can convert it to a graph and then apply GNNs} the majority of these methods are highly limited since their models ignore the high-order structural information in observed data. For example, the optimization goal of the GEX-ADT prediction task is to predict ADT features (i.e. the number of proteins in each cell captured by Antibody-Derived Tags), and the input of the training samples is the GEX features (i.e. the number of unique molecular identifiers [UMI] in each cell). During the parameter updating for a specific cell, only the UMIs identified in itself are involved. Besides, noise and sparsity are long-existing substantial hurdles in analyzing single-cell data~\cite{lahnemann2020eleven}, furthermore, integrated measuring often require additional processing to cells, which is a non-trivial work and can lead to extra noise and drop-out in the resulting data~\cite{lee2020single, mimitou2021scalable}, therefore, it would be very essential to introduce some extra smoothing techniques.

\jt{Next we discuss the advance of GNNs, and why GNNs are suitable to these tasks and what are the advantages? So there are works applying GNNs in single-cell analysis that demonstrate the potentials of GNNs in the tasks for the competition. We just need to mention we develop GNNs for these tasks and we can add a footnote to mention our solution won the first place and so on}

Recently, the advances of graph neural networks pave the way for addressing above issues in single-cell data integration. Specifically, graph neural networks aggregate embedding from neighborhood iteratively. Thus, throughout the propagation layers, the node embedding can eventually encode high-order structural information, which is different from the previous models which only capture first-order local information. Besides, graph neural networks naturally smooth the features by aggregating neighbors' embedding, which provides an extra denoising effect other than previous methods. There are even more advantages for using graph neural networks in single-cell data integration, for example, it is very natural to incorporate external knowledge (e.g. correlations between genes) into the constructed graph and apply graph neural networks to exploit the additional structural information. Another good feature of graph neural networks is its transductive learning paradigm, which can help us gain additional semi-supervised signal to enhance the representation learning process.

In view of such advantages of graph neural networks, several existing works attempted to introduce graph neural networks to single cell analysis, such as~\cite{song2021scgcn,wang2021scgnn,ciortan2022gnn,shao2021scdeepsort}, however, they focused on very different tasks and none of them is related to multimodal integration. Therefore, we decided to explore our own methods to apply graph neural networks to these multimodal tasks, and we were lucky to get the first place in the overall ranking of modality prediction task in the Multimodal Single-Cell Data Integration competition. 

After the competition, we continued working on the topic and eventually we designed three different models for the three tasks of the competition. These models share the general framework but have different characteristics. To the best of our knowledge, we are the first one to propose a graph neural networks (GNN) framework in this emerging research topic (a.k.a  multimodal single-cell data integration), and our models achieve the best results in all of these three new tasks, providing a very strong baseline for follow-up research. Our contributions can be summarized as follows:
\begin{itemize}
	\item We propose a general framework for utilizing graph neural networks in multimodal single-cell data integration tasks and verified its feasibility in three different new problems.
	\item We provide a novel cross-modality translation GNN model which can naturally incorporate domain knowledge, and a practical modality matching GNN model which is very scalable to high dimensional modality.
	\item Our models achieve very high performance, winning the first place in the overall ranking of modality prediction task in the Multimodal Single-Cell Data Integration competition, and currently surpassing every model for every task on the leaderboard. All of our results are based on publicly available data and have perfect reproducibility.
	
\end{itemize}


\hongzhi{@Wei: 'challenges' are very weak; 'to address....we propose....' is also hard to write, because we have different models for different tasks, and our main exploration is in task1, but we cannot focus on task1 here. I suggest to write as above\\}
%In fact, graph neural networks for multimodal integration have to pay attention to some special issues: (1) scalability issue, since data in some modalities could have very large feature dimensions (e.g. ATAC-seq feature have more than 110,000 dimensions), (2) prior knowledge modeling, some prior knowledge is very useful for these tasks, especially considering that the amount of aligned data is very limited.



The rest of the paper is organized as follows. We explain the three new problems in Section 2. We define our general framework and model specifications in Section 3. Experimental setup and results are illustrated and analyzed in Section 4. Related works are reviewed in Section 5. We conclude the paper in Section 6.

% \newpage
